Automated Graph Machine Learning: Approaches, Libraries, Benchmarks and Directions

Graph machine learning has been extensively studied in both academic and industry. However, as the literature on graph learning booms with a vast number of emerging methods and techniques, it becomes increasingly difficult to manually design the optimal machine learning algorithm for different graph-related tasks. To tackle the challenge, automated graph machine learning, which aims at discovering the best hyper-parameter and neural architecture configuration for different graph tasks/data without manual design, is gaining an increasing number of attentions from the research community. In this paper, we extensively discuss automated graph machine learning approaches, covering hyper-parameter optimization (HPO) and neural architecture search (NAS) for graph machine learning. We briefly overview existing libraries designed for either graph machine learning or automated machine learning respectively, and further in depth introduce AutoGL, our dedicated and the world's first open-source library for automated graph machine learning. Also, we describe a tailored benchmark that supports unified, reproducible, and efficient evaluations. Last but not least, we share our insights on future research directions for automated graph machine learning. This paper is the first systematic and comprehensive discussion of approaches, libraries as well as directions for automated graph machine learning.

==> autogr-ref.tex <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{100}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{newman2018networks}
M.~Newman, \emph{Networks}.\hskip 1em plus 0.5em minus 0.4em\relax Oxford
  university press, 2018.

\bibitem{cui2018survey}
P.~Cui, X.~Wang, J.~Pei, and W.~Zhu, ``A survey on network embedding,''
  \emph{IEEE transactions on knowledge and data engineering}, vol.~31, no.~5,
  pp. 833--852, 2018.

\bibitem{hamilton2017representation}
W.~L. Hamilton, R.~Ying, and J.~Leskovec, ``Representation learning on graphs:
  Methods and applications,'' \emph{IEEE DEBU}, 2017.

\bibitem{goyal2018graph}
P.~Goyal and E.~Ferrara, ``Graph embedding techniques, applications, and
  performance: A survey,'' \emph{KBS}, 2018.

\bibitem{cai2018comprehensive}
H.~Cai, V.~W. Zheng, and K.~C.-C. Chang, ``A comprehensive survey of graph
  embedding: Problems, techniques, and applications,'' \emph{TKDE}, 2018.

\bibitem{zhang2020deep}
Z.~Zhang, P.~Cui, and W.~Zhu, ``Deep learning on graphs: A survey,''
  \emph{TKDE}, 2020.

\bibitem{wu2020comprehensive}
Z.~Wu \emph{et~al.}, ``A comprehensive survey on graph neural networks,''
  \emph{TNNLS}, 2020.

\bibitem{zhou2018graph}
J.~Zhou \emph{et~al.}, ``Graph neural networks: A review of methods and
  applications,'' \emph{arXiv:1812.08434}, 2018.

\bibitem{ying2018graph}
R.~Ying \emph{et~al.}, ``Graph convolutional neural networks for web-scale
  recommender systems,'' in \emph{KDD}, 2018.

\bibitem{ma2019learning}
J.~Ma \emph{et~al.}, ``Learning disentangled representations for
  recommendation,'' in \emph{NeurIPS}, 2019.

\bibitem{li2021intention}
H.~Li, X.~Wang, Z.~Zhang, J.~Ma, P.~Cui, and W.~Zhu, ``Intention-aware
  sequential recommendation with structured intent transition,'' \emph{IEEE
  Transactions on Knowledge and Data Engineering}, vol.~34, no.~11, pp.
  5403--5414, 2021.

\bibitem{liu2023graph}
S.~Liu, Z.~Meng, C.~Macdonald, and I.~Ounis, ``Graph neural pre-training for
  recommendation with side information,'' \emph{ACM Transactions on Information
  Systems}, vol.~41, no.~3, pp. 1--28, 2023.

\bibitem{cui2022can}
H.~Cui, J.~Lu, Y.~Ge, and C.~Yang, ``How can graph neural networks help
  document retrieval: A case study on cord19 with concept map generation,'' in
  \emph{European Conference on Information Retrieval}.\hskip 1em plus 0.5em
  minus 0.4em\relax Springer, 2022, pp. 75--83.

\bibitem{feng2022dc}
C.~Feng, Y.~He, S.~Wen, G.~Liu, L.~Wang, J.~Xu, and B.~Zheng, ``Dc-gnn:
  Decoupled graph neural networks for improving and accelerating large-scale
  e-commerce retrieval,'' in \emph{Companion Proceedings of the Web Conference
  2022}, 2022, pp. 32--40.

\bibitem{wang2022gnn}
L.~Wang, X.~Li, H.~Zhang, Y.~Dai, and S.~Zhang, ``Gnn-based retrieval and
  recommadation system: A semantic enhenced graph model,'' in \emph{2022 IEEE
  5th Advanced Information Management, Communicates, Electronic and Automation
  Control Conference (IMCEC)}, vol.~5.\hskip 1em plus 0.5em minus 0.4em\relax
  IEEE, 2022, pp. 1823--1830.

\bibitem{liang2023abslearn}
K.~Liang, J.~Tan, D.~Zeng, Y.~Huang, X.~Huang, and G.~Tan, ``Abslearn: a
  gnn-based framework for aliasing and buffer-size information retrieval,''
  \emph{Pattern Analysis and Applications}, pp. 1--19, 2023.

\bibitem{akoglu2015graph}
L.~Akoglu, H.~Tong, and D.~Koutra, ``Graph based anomaly detection and
  description: a survey,'' \emph{DMKD}, 2015.

\bibitem{su2020network}
C.~Su \emph{et~al.}, ``Network embedding in biomedical data science,''
  \emph{Briefings in bioinformatics}, 2020.

\bibitem{zitnik2017predicting}
M.~Zitnik and J.~Leskovec, ``Predicting multicellular function through
  multi-layer tissue networks,'' \emph{Bioinformatics}, 2017.

\bibitem{kipf2018neural}
T.~Kipf \emph{et~al.}, ``Neural relational inference for interacting systems,''
  \emph{ICML}, 2018.

\bibitem{li2018dcrnn_traffic}
Y.~Li \emph{et~al.}, ``Diffusion convolutional recurrent neural network:
  Data-driven traffic forecasting,'' in \emph{ICLR}, 2018.

\bibitem{yu2018spatio}
B.~Yu, H.~Yin, and Z.~Zhu, ``Spatio-temporal graph convolutional networks: a
  deep learning framework for traffic forecasting,'' in \emph{IJCAI}, 2018.

\bibitem{wang2017knowledge}
Q.~Wang \emph{et~al.}, ``Knowledge graph embedding: A survey of approaches and
  applications,'' \emph{TKDE}, 2017.

\bibitem{ioannidis2020few}
V.~N. Ioannidis, D.~Zheng, and G.~Karypis, ``Few-shot link prediction via graph
  neural networks for covid-19 drug-repurposing,'' \emph{arXiv:2007.10261},
  2020.

\bibitem{gysi2020network}
D.~M. Gysi \emph{et~al.}, ``Network medicine framework for identifying drug
  repurposing opportunities for covid-19,'' \emph{arXiv:2004.07229}, 2020.

\bibitem{kapoor2020examining}
A.~Kapoor \emph{et~al.}, ``Examining covid-19 forecasting using spatio-temporal
  graph neural networks,'' \emph{arXiv:2007.03113}, 2020.

\bibitem{he2020automl}
X.~He, K.~Zhao, and X.~Chu, ``Automl: A survey of the state-of-the-art,''
  \emph{KBS}, 2020.

\bibitem{yao2018taking}
Q.~Yao, M.~Wang, Y.~Chen, W.~Dai, Y.-F. Li, W.-W. Tu, Q.~Yang, and Y.~Yu,
  ``Taking human out of learning applications: A survey on automated machine
  learning,'' \emph{arXiv:1810.13306}, 2018.

\bibitem{bergstra2012random}
J.~Bergstra and Y.~Bengio, ``Random search for hyper-parameter optimization,''
  \emph{JMLR}, 2012.

\bibitem{bergstra2011algorithms}
J.~Bergstra \emph{et~al.}, ``Algorithms for hyper-parameter optimization,''
  \emph{NeurIPS}, 2011.

\bibitem{snoek2012practical}
J.~Snoek, H.~Larochelle, and R.~P. Adams, ``Practical bayesian optimization of
  machine learning algorithms,'' \emph{NeurIPS}, 2012.

\bibitem{liu2021meta}
Y.~Liu, X.~Wang, X.~Xu, J.~Yang, and W.~Zhu, ``Meta hyperparameter optimization
  with adversarial proxy subsets sampling,'' in \emph{Proceedings of the 30th
  ACM International Conference on Information \& Knowledge Management}, 2021,
  pp. 1109--1118.

\bibitem{elsken2019neural}
T.~Elsken, J.~H. Metzen, and F.~Hutter, ``Neural architecture search: A
  survey,'' \emph{JMLR}, 2019.

\bibitem{wei2021autoias}
Z.~Wei, X.~Wang, and W.~Zhu, ``Autoias: Automatic integrated architecture
  searcher for click-trough rate prediction,'' in \emph{Proceedings of the 30th
  ACM International Conference on Information \& Knowledge Management}, 2021,
  pp. 2101--2110.

\bibitem{zoph2017neural}
B.~Zoph and Q.~V. Le, ``Neural architecture search with reinforcement
  learning,'' in \emph{ICLR}, 2017.

\bibitem{liu2018darts}
H.~Liu, K.~Simonyan, and Y.~Yang, ``Darts: Differentiable architecture
  search,'' in \emph{ICLR}, 2018.

\bibitem{pham2018efficient}
H.~Pham \emph{et~al.}, ``Efficient neural architecture search via parameters
  sharing,'' in \emph{ICML}, 2018.

\bibitem{zoph2018learning}
B.~Zoph \emph{et~al.}, ``Learning transferable architectures for scalable image
  recognition,'' in \emph{CVPR}, 2018.

\bibitem{real2019regularized}
E.~Real \emph{et~al.}, ``Regularized evolution for image classifier
  architecture search,'' in \emph{AAAI}, 2019.

\bibitem{gilmer2017neural}
J.~Gilmer \emph{et~al.}, ``Neural message passing for quantum chemistry,'' in
  \emph{ICML}, 2017.

\bibitem{bronstein2017geometric}
M.~M. Bronstein \emph{et~al.}, ``Geometric deep learning: going beyond
  euclidean data,'' \emph{IEEE Signal Processing Magazine}, 2017.

\bibitem{ijcai2020-195}
Y.~Gao \emph{et~al.}, ``Graph neural architecture search,'' in \emph{IJCAI},
  2020.

\bibitem{hu2020open}
W.~Hu \emph{et~al.}, ``Open graph benchmark: Datasets for machine learning on
  graphs,'' \emph{NeurIPS}, 2020.

\bibitem{zang2018power}
C.~Zang \emph{et~al.}, ``On power law growth of social networks,'' \emph{TKDE},
  2018.

\bibitem{tu2019autone}
K.~Tu \emph{et~al.}, ``Autone: Hyperparameter optimization for massive network
  embedding,'' in \emph{KDD}, 2019.

\bibitem{wang2021explainable}
X.~Wang \emph{et~al.}, ``Explainable automated graph representation learning
  with hyperparameter importance,'' in \emph{ICML}, 2021.

\bibitem{zhang2018arbitrary}
Z.~Zhang \emph{et~al.}, ``Arbitrary-order proximity preserved network
  embedding,'' in \emph{KDD}, 2018.

\bibitem{perozzi2014deepwalk}
B.~Perozzi, R.~Al-Rfou, and S.~Skiena, ``Deepwalk: Online learning of social
  representations,'' in \emph{KDD}, 2014.

\bibitem{kipf2017semi}
T.~N. Kipf and M.~Welling, ``Semi-supervised classification with graph
  convolutional networks,'' in \emph{ICLR}, 2017.

\bibitem{guo2021jitune}
M.~Guo \emph{et~al.}, ``Jitune: Just-in-time hyperparameter tuning for network
  embedding algorithms,'' \emph{arXiv:2101.06427}, 2021.

\bibitem{yuan2021novel}
Y.~Yuan \emph{et~al.}, ``A novel genetic algorithm with hierarchical evaluation
  strategy for hyperparameter optimisation of graph neural networks,''
  \emph{arXiv:2101.09300}, 2021.

\bibitem{yoon2020autonomous}
M.~Yoon \emph{et~al.}, ``Autonomous graph mining algorithm search with best
  speed/accuracy trade-off,'' in \emph{IEEE ICDM}, 2020.

\bibitem{yuan2021hyperparameters}
Y.~Yuan, W.~Wang, and W.~Pang, ``Which hyperparameters to optimise? an
  investigation of evolutionary hyperparameter optimisation in graph neural
  network for molecular property prediction,'' in \emph{GECCO}, 2021.

\bibitem{yuan2021systematic}
------, ``A systematic comparison study on hyperparameter optimisation of graph
  neural networks for molecular property prediction,'' in \emph{GECCO}, 2021.

\bibitem{zhu2021automated}
R.~Zhu, Z.~Tao, Y.~Li, and S.~Li, ``Automated graph learning via population
  based self-tuning gcn,'' in \emph{Proceedings of the 44th International ACM
  SIGIR Conference on Research and Development in Information Retrieval}, 2021,
  pp. 2096--2100.

\bibitem{bu2021automatic}
C.~Bu, Y.~Lu, and F.~Liu, ``Automatic graph learning with evolutionary
  algorithms: An experimental study,'' in \emph{PRICAI}, 2021.

\bibitem{sun2021automated}
J.~Sun, B.~Wang, and B.~Wu, ``Automated graph representation learning for node
  classification,'' in \emph{IJCNN}, 2021.

\bibitem{yang2022calibrate}
X.~Yang, J.~Wang, X.~Zhao, S.~Li, and Z.~Tao, ``Calibrate automated graph
  neural network via hyperparameter uncertainty,'' in \emph{Proceedings of the
  31st ACM International Conference on Information \& Knowledge Management},
  2022, pp. 4640--4644.

\bibitem{lloyd2023assessing}
O.~Lloyd, Y.~Liu, and T.~R~Gaunt, ``Assessing the effects of hyperparameters on
  knowledge graph embedding quality,'' \emph{Journal of big Data}, vol.~10,
  no.~1, pp. 1--15, 2023.

\bibitem{yoon2022autonomous}
M.~Yoon, T.~Gervet, B.~Hooi, and C.~Faloutsos, ``Autonomous graph mining
  algorithm search with best performance trade-off,'' \emph{Knowledge and
  Information Systems}, vol.~64, no.~6, pp. 1571--1602, 2022.

\bibitem{zhang2022kgtuner}
Y.~Zhang, Z.~Zhou, Q.~Yao, and Y.~Li, ``Kgtuner: Efficient hyper-parameter
  search for knowledge graph learning,'' \emph{arXiv preprint
  arXiv:2205.02460}, 2022.

\bibitem{yang2022revisiting}
D.~Yang, B.~Qu, R.~Hussein, P.~Rosso, P.~Cudr{\'e}-Mauroux, and J.~Liu,
  ``Revisiting embedding based graph analyses: Hyperparameters matter!''
  \emph{IEEE Transactions on Knowledge and Data Engineering}, 2022.

\bibitem{zhou2019auto}
K.~Zhou \emph{et~al.}, ``Auto-gnn: Neural architecture search of graph neural
  networks,'' \emph{arXiv:1909.03184}, 2019.

\bibitem{zhao2020simplifying}
H.~Zhao, L.~Wei, and Q.~Yao, ``Simplifying architecture search for graph neural
  network,'' \emph{arXiv:2008.11652}, 2020.

\bibitem{zhao2020probabilistic}
Y.~Zhao \emph{et~al.}, ``Probabilistic dual network architecture search on
  graphs,'' \emph{arXiv:2003.09676}, 2020.

\bibitem{nunes2020neural}
M.~Nunes \emph{et~al.}, ``Neural architecture search in graph neural
  networks,'' in \emph{Brazilian Conference on Intelligent Systems}, 2020.

\bibitem{li2020autograph}
Y.~Li and I.~King, ``Autograph: Automated graph neural network,'' in
  \emph{ICONIP}, 2020.

\bibitem{shi2020evolutionary}
M.~Shi \emph{et~al.}, ``Evolutionary architecture search for graph neural
  networks,'' \emph{arXiv:2009.10199}, 2020.

\bibitem{zhao2021efficient}
\BIBentryALTinterwordspacing
H.~Zhao \emph{et~al.}, ``Efficient graph neural architecture search,'' 2021.
  [Online]. Available: \url{https://openreview.net/forum?id=IjIzIOkK2D6}
\BIBentrySTDinterwordspacing

\bibitem{jiang2020graph}
S.~Jiang and P.~Balaprakash, ``Graph neural network architecture search for
  molecular property prediction,'' in \emph{IEEE Big Data}, 2020.

\bibitem{zhao2020learned}
Y.~Zhao \emph{et~al.}, ``Learned low precision graph neural networks,'' in
  \emph{EuroMLSys}, 2021.

\bibitem{you2020design}
J.~You, Z.~Ying, and J.~Leskovec, ``Design space for graph neural networks,''
  \emph{NeurIPS}, 2020.

\bibitem{li2020sgas}
G.~Li \emph{et~al.}, ``Sgas: Sequential greedy architecture search,'' in
  \emph{CVPR}, 2020.

\bibitem{peng2020learning}
W.~Peng \emph{et~al.}, ``Learning graph convolutional network for
  skeleton-based human action recognition by neural searching,'' \emph{AAAI},
  2020.

\bibitem{pourchot2018cemrl}
Pourchot and Sigaud, ``{CEM}-{RL}: Combining evolutionary and gradient-based
  methods for policy search,'' in \emph{ICLR}, 2019.

\bibitem{cai2021rethinking}
S.~Cai \emph{et~al.}, ``Rethinking graph neural architecture search from
  message-passing,'' \emph{CVPR}, 2021.

\bibitem{pan2021autostg}
Z.~Pan \emph{et~al.}, ``Autostg: Neural architecture search for predictions of
  spatio-temporal graphs,'' \emph{WWW}, 2021.

\bibitem{li2021one}
Y.~Li \emph{et~al.}, ``One-shot graph neural architecture search with dynamic
  search space,'' \emph{AAAI}, 2021.

\bibitem{zhao2021search}
H.~Zhao, Q.~Yao, and W.~Tu, ``Search to aggregate neighborhood for graph neural
  network,'' \emph{ICDE}, 2021.

\bibitem{guan2021autoattend}
C.~Guan, X.~Wang, and W.~Zhu, ``Autoattend: Automated attention representation
  search,'' in \emph{ICML}, 2021.

\bibitem{ding2020propagation}
Y.~Ding \emph{et~al.}, ``Diffmg: Differentiable meta graph search for
  heterogeneous graph neural networks,'' in \emph{KDD}, 2021.

\bibitem{feng2021search}
G.~Feng, C.~Wang, and H.~Wang, ``Search for deep graph neural networks,''
  \emph{arXiv:2109.10047}, 2021.

\bibitem{wei2021learn}
L.~Wei, H.~Zhao, and Z.~He, ``Learn layer-wise connections in graph neural
  networks,'' \emph{arXiv:2112.13585}, 2021.

\bibitem{wang2021fl}
C.~Wang \emph{et~al.}, ``Fl-agcns: Federated learning framework for automatic
  graph convolutional network search,'' \emph{arXiv:2104.04141}, 2021.

\bibitem{zhang2021g}
Y.~Zhang, H.~You, Y.~Fu, T.~Geng, A.~Li, and Y.~Lin, ``G-cos: Gnn-accelerator
  co-search towards both better accuracy and efficiency,'' in \emph{2021
  IEEE/ACM International Conference On Computer Aided Design (ICCAD)}.\hskip
  1em plus 0.5em minus 0.4em\relax IEEE, 2021, pp. 1--9.

\bibitem{wei2021pooling}
L.~Wei, H.~Zhao, Q.~Yao, and Z.~He, ``Pooling architecture search for graph
  classification,'' in \emph{Proceedings of the 30th ACM International
  Conference on Information \& Knowledge Management}, 2021, pp. 2091--2100.

\bibitem{lu2020fgnas}
Q.~Lu, W.~Jiang, M.~Jiang, J.~Hu, S.~Dasgupta, and Y.~Shi, ``Fgnas: Fpga-aware
  graph neural architecture search,'' 2020.

\bibitem{chen2021graphpas}
J.~Chen \emph{et~al.}, ``Graphpas: Parallel architecture search for graph
  neural networks,'' in \emph{SIGIR}, 2021.

\bibitem{cai2021algnn}
R.~Cai \emph{et~al.}, ``Algnn: Auto-designed lightweight graph neural
  network,'' in \emph{PRICAI}, 2021.

\bibitem{coello2002mopso}
C.~C. Coello and M.~S. Lechuga, ``Mopso: A proposal for multiple objective
  particle swarm optimization,'' in \emph{CEC}, 2002.

\bibitem{cai2021edge}
S.~Cai \emph{et~al.}, ``Edge-featured graph neural architecture search,''
  \emph{arXiv:2109.01356}, 2021.

\bibitem{wang2021autogel}
Z.~Wang, S.~Di, and L.~Chen, ``Autogel: An automated graph neural network with
  explicit link information,'' \emph{NeurIPS}, 2021.

\bibitem{xie2019snas}
S.~Xie \emph{et~al.}, ``Snas: stochastic neural architecture search,''
  \emph{ICLR}, 2019.

\bibitem{qin2021graph}
Y.~Qin, X.~Wang, Z.~Zhang, and W.~Zhu, ``Graph differentiable architecture
  search with structure learning,'' \emph{Advances in neural information
  processing systems}, vol.~34, pp. 16\,860--16\,872, 2021.

\bibitem{xie2023adversarially}
B.~Xie, H.~Chang, Z.~Zhang, X.~Wang, D.~Wang, Z.~Zhang, R.~Ying, and W.~Zhu,
  ``Adversarially robust neural architecture search for graph neural
  networks,'' in \emph{Proceedings of the IEEE/CVF Conference on Computer
  Vision and Pattern Recognition}, 2023, pp. 8143--8152.

\bibitem{qin2022graph}
Y.~Qin, X.~Wang, Z.~Zhang, P.~Xie, and W.~Zhu, ``Graph neural architecture
  search under distribution shifts,'' in \emph{International Conference on
  Machine Learning}.\hskip 1em plus 0.5em minus 0.4em\relax PMLR, 2022, pp.
  18\,083--18\,095.

\bibitem{guan2022large}
C.~Guan, X.~Wang, H.~Chen, Z.~Zhang, and W.~Zhu, ``Large-scale graph neural
  architecture search,'' in \emph{International Conference on Machine
  Learning}.\hskip 1em plus 0.5em minus 0.4em\relax PMLR, 2022, pp. 7968--7981.

\bibitem{zhang2022pasca}
W.~Zhang, Y.~Shen, Z.~Lin, Y.~Li, X.~Li, W.~Ouyang, Y.~Tao, Z.~Yang, and
  B.~Cui, ``Pasca: A graph neural architecture search system under the scalable
  paradigm,'' in \emph{Proceedings of the ACM Web Conference 2022}, 2022, pp.
  1817--1828.

\bibitem{li2023differentiable}
C.~Li, H.~Xu, and K.~He, ``Differentiable meta multigraph search with partial
  message propagation on heterogeneous information networks,'' in
  \emph{Proceedings of the AAAI Conference on Artificial Intelligence},
  vol.~37, no.~7, 2023, pp. 8518--8526.

\bibitem{zhang2023dynamic}
Z.~Zhang, Z.~Zhang, X.~Wang, Y.~Qin, Z.~Qin, and W.~Zhu, ``Dynamic
  heterogeneous graph attention neural architecture search,'' \emph{AAAI},
  2023.

\bibitem{li2019deepgcns}
G.~Li \emph{et~al.}, ``Deepgcns: Can gcns go as deep as cnns?'' in \emph{ICCV},
  2019.

\bibitem{xu2018representation}
K.~Xu \emph{et~al.}, ``Representation learning on graphs with jumping knowledge
  networks,'' in \emph{ICML}, 2018.

\bibitem{ying2018hierarchical}
R.~Ying \emph{et~al.}, ``Hierarchical graph representation learning with
  differentiable pooling,'' in \emph{NeurIPS}, 2018.

\bibitem{li2018deeper}
Q.~Li, Z.~Han, and X.-M. Wu, ``Deeper insights into graph convolutional
  networks for semi-supervised learning,'' in \emph{AAAI}, 2018.

\bibitem{jang2017categorical}
E.~Jang, S.~Gu, and B.~Poole, ``Categorical reparameterization with
  gumbel-softmax,'' in \emph{ICLR}, 2017.

\bibitem{maddison2017concrete}
C.~J. Maddison, A.~Mnih, and Y.~W. Teh, ``The concrete distribution: A
  continuous relaxation of discrete random variables,'' in \emph{ICLR}, 2017.

\bibitem{shi2020bridging}
H.~Shi \emph{et~al.}, ``Bridging the gap between sample-based and one-shot
  neural architecture search with bonas,'' \emph{NeurIPS}, 2020.

\bibitem{guo2020single}
Z.~Guo \emph{et~al.}, ``Single path one-shot neural architecture search with
  uniform sampling,'' in \emph{ECCV}, 2020.

\bibitem{real2017large}
E.~Real \emph{et~al.}, ``Large-scale evolution of image classifiers,'' in
  \emph{ICML}, 2017.

\bibitem{li2021disentangled}
H.~Li, X.~Wang, Z.~Zhang, Z.~Yuan, H.~Li, and W.~Zhu, ``Disentangled
  contrastive learning on graphs,'' \emph{Advances in Neural Information
  Processing Systems}, vol.~34, pp. 21\,872--21\,884, 2021.

\bibitem{li2022disentangled}
H.~Li, Z.~Zhang, X.~Wang, and W.~Zhu, ``Disentangled graph contrastive learning
  with independence promotion,'' \emph{IEEE Transactions on Knowledge and Data
  Engineering}, 2022.

\bibitem{ding2021diffmg}
Y.~Ding, Q.~Yao, H.~Zhao, and T.~Zhang, ``Diffmg: Differentiable meta graph
  search for heterogeneous graph neural networks,'' in \emph{Proceedings of the
  27th ACM SIGKDD Conference on Knowledge Discovery \& Data Mining}, 2021, pp.
  279--288.

\bibitem{gao2023hgnaspp}
Y.~Gao, P.~Zhang, C.~Zhou, H.~Yang, Z.~Li, Y.~Hu, and S.~Y. Philip, ``Hgnas++:
  efficient architecture search for heterogeneous graph neural networks,''
  \emph{IEEE Transactions on Knowledge and Data Engineering}, 2023.

\bibitem{zhang2023autogt}
\BIBentryALTinterwordspacing
Z.~Zhang, X.~Wang, C.~Guan, Z.~Zhang, H.~Li, and W.~Zhu, ``Auto{GT}: Automated
  graph transformer architecture search,'' in \emph{The Eleventh International
  Conference on Learning Representations}, 2023. [Online]. Available:
  \url{https://openreview.net/forum?id=GcM7qfl5zY}
\BIBentrySTDinterwordspacing

\bibitem{ying2021do}
\BIBentryALTinterwordspacing
C.~Ying, T.~Cai, S.~Luo, S.~Zheng, G.~Ke, D.~He, Y.~Shen, and T.-Y. Liu, ``Do
  transformers really perform badly for graph representation?'' in
  \emph{Advances in Neural Information Processing Systems}, A.~Beygelzimer,
  Y.~Dauphin, P.~Liang, and J.~W. Vaughan, Eds., 2021. [Online]. Available:
  \url{https://openreview.net/forum?id=OeWooOxFwDa}
\BIBentrySTDinterwordspacing

\bibitem{you2020graph}
J.~You \emph{et~al.}, ``Graph structure of neural networks,'' in \emph{ICML},
  2020.

\bibitem{Fey2019fast}
M.~Fey and J.~E. Lenssen, ``Fast graph representation learning with {PyTorch
  Geometric},'' in \emph{ICLR Workshop}, 2019.

\bibitem{dgl}
M.~Wang, D.~Zheng, Z.~Ye, Q.~Gan, M.~Li, X.~Song, J.~Zhou, C.~Ma, L.~Yu, Y.~Gai
  \emph{et~al.}, ``Deep graph library: A graph-centric, highly-performant
  package for graph neural networks,'' \emph{arXiv preprint arXiv:1909.01315},
  2019.

\bibitem{graphnet}
P.~W. Battaglia \emph{et~al.}, ``Relational inductive biases, deep learning,
  and graph networks,'' \emph{arXiv:1806.01261}, 2018.

\bibitem{aligraph}
R.~Zhu \emph{et~al.}, ``Aligraph: A comprehensive graph neural network
  platform,'' \emph{VLDB}, 2019.

\bibitem{euler}
Alibaba, ``Euler: A distributed graph deep learning framework,''
  \url{https://github.com/alibaba/euler}, 2019.

\bibitem{pbg}
A.~Lerer \emph{et~al.}, ``{PyTorch-BigGraph: A Large-scale Graph Embedding
  System},'' in \emph{SysML}, 2019.

\bibitem{pgl}
NLP and P.~T. at~Baidu, ``Paddle graph learning,''
  \url{https://github.com/PaddlePaddle/PGL}, 2021, [Online; accessed
  28-Dec-2021].

\bibitem{tfgnn}
J.~P. Sibon~Li \emph{et~al.}, ``Tensorflow gnn,''
  \url{https://github.com/tensorflow/gnn}, 2021, [Online; accessed
  28-Dec-2021].

\bibitem{StellarGraph}
C.~Data61, ``Stellargraph machine learning library,''
  \url{https://github.com/stellargraph/stellargraph}, 2018.

\bibitem{spektral}
D.~Grattarola and C.~Alippi, ``Graph neural networks in tensorflow and keras
  with spektral,'' \emph{ICML workshop}, 2020.

\bibitem{cogdl}
T.~U. Knowledge Engineering~Group, ``Cogdl: An extensive research toolkit for
  deep learning on graphs,'' \url{https://github.com/THUDM/cogdl}, 2020.

\bibitem{openne}
N.~L. P.~L. at~Tsinghua~University, ``Openne: An open source toolkit for
  network embedding,'' \url{https://github.com/thunlp/OpenNE}, 2018.

\bibitem{openhgnn}
O.~T. at~GAMMA~LAB and D.~Team, ``Heterogeneous graph neural network,''
  \url{https://github.com/BUPT-GAMMA/OpenHGNN}, 2021, [Online; accessed
  28-Dec-2021].

\bibitem{gem}
P.~Goyal and E.~Ferrara, ``Gem: A python package for graph embedding methods,''
  \emph{JOSS}, 2018.

\bibitem{karateclub}
B.~Rozemberczki, O.~Kiss, and R.~Sarkar, ``{Karate Club: An API Oriented
  Open-source Python Framework for Unsupervised Learning on Graphs},'' in
  \emph{CIKM}, 2020.

\bibitem{hagberg2008exploring}
A.~Hagberg, P.~Swart, and D.~S~Chult, ``Exploring network structure, dynamics,
  and function using networkx,'' Los Alamos National Lab.(LANL), Tech. Rep.,
  2008.

\bibitem{nni}
Q.~Zhang \emph{et~al.}, ``Retiarii: A deep learning exploratory-training
  framework,'' in \emph{OSDI}, 2020.

\bibitem{autokeras}
H.~Jin, Q.~Song, and X.~Hu, ``Auto-keras: An efficient neural architecture
  search system,'' in \emph{KDD}, 2019.

\bibitem{autosklearn}
M.~Feurer \emph{et~al.}, ``Auto-sklearn: efficient and robust automated machine
  learning,'' in \emph{Automated Machine Learning}, 2019.

\bibitem{hyperopt}
J.~Bergstra, D.~Yamins, and D.~Cox, ``Making a science of model search:
  Hyperparameter optimization in hundreds of dimensions for vision
  architectures,'' in \emph{ICML}, 2013.

\bibitem{tpot}
R.~S. Olson \emph{et~al.}, ``Evaluation of a tree-based pipeline optimization
  tool for automating data science,'' in \emph{GECCO}, 2016.

\bibitem{agtabular}
N.~Erickson \emph{et~al.}, ``Autogluon-tabular: Robust and accurate automl for
  structured data,'' \emph{arXiv:2003.06505}, 2020.

\bibitem{mlbox}
A.~de~Romblay \emph{et~al.}, ``Mlbox, machine learning box,''
  \url{https://github.com/AxeldeRomblay/MLBox}, 2018.

\bibitem{mljar}
MLJAR, ``Mljar automated machine learning,''
  \url{https://github.com/mljar/mljar-supervised}, 2019.

\bibitem{sen2008collective}
P.~Sen \emph{et~al.}, ``Collective classification in network data,'' \emph{AI
  magazine}, 2008.

\bibitem{shchur2018pitfalls}
O.~Shchur \emph{et~al.}, ``Pitfalls of graph neural network evaluation,''
  \emph{Relational Representation Learning Workshop, NeurIPS 2018}, 2018.

\bibitem{hamilton2017inductive}
W.~Hamilton, Z.~Ying, and J.~Leskovec, ``Inductive representation learning on
  large graphs,'' in \emph{NeurIPS}, 2017.

\bibitem{mutag}
A.~K. Debnath, R.~L. Lopez~de Compadre, G.~Debnath, A.~J. Shusterman, and
  C.~Hansch, ``Structure-activity relationship of mutagenic aromatic and
  heteroaromatic nitro compounds. correlation with molecular orbital energies
  and hydrophobicity,'' \emph{Journal of medicinal chemistry}, vol.~34, no.~2,
  pp. 786--797, 1991.

\bibitem{borgwardt2005protein}
K.~M. Borgwardt \emph{et~al.}, ``Protein function prediction via graph
  kernels,'' \emph{Bioinformatics}, 2005.

\bibitem{graphkernel}
P.~Yanardag and S.~Vishwanathan, ``Deep graph kernels,'' in \emph{KDD}, 2015.

\bibitem{milo2002network}
R.~Milo, S.~Shen-Orr, S.~Itzkovitz, N.~Kashtan, D.~Chklovskii, and U.~Alon,
  ``Network motifs: simple building blocks of complex networks,''
  \emph{Science}, vol. 298, no. 5594, pp. 824--827, 2002.

\bibitem{zhang2021eigen}
Z.~Zhang, P.~Cui, J.~Pei, X.~Wang, and W.~Zhu, ``Eigen-gnn: A graph structure
  preserving plug-in for gnns,'' \emph{IEEE Transactions on Knowledge and Data
  Engineering}, 2021.

\bibitem{pagerank}
S.~Brin and L.~Page, ``The anatomy of a large-scale hypertextual web search
  engine,'' \emph{Computer networks and ISDN systems}, 1998.

\bibitem{NIPS2017_6449f44a}
G.~Ke, Q.~Meng, T.~Finley, T.~Wang, W.~Chen, W.~Ma, Q.~Ye, and T.-Y. Liu,
  ``Lightgbm: A highly efficient gradient boosting decision tree,''
  \emph{Advances in neural information processing systems}, vol.~30, 2017.

\bibitem{rossi2018deep}
R.~A. Rossi, R.~Zhou, and N.~K. Ahmed, ``Deep inductive graph representation
  learning,'' \emph{TKDE}, 2018.

\bibitem{tsitsulin2018netlsd}
A.~Tsitsulin, D.~Mottin, P.~Karras, A.~Bronstein, and E.~M{\"u}ller, ``Netlsd:
  hearing the shape of a graph,'' in \emph{Proceedings of the 24th ACM SIGKDD
  International Conference on Knowledge Discovery \& Data Mining}, 2018, pp.
  2347--2356.

\bibitem{velickovic2018graph}
P.~Veli{\v{c}}kovi{\'{c}} \emph{et~al.}, ``{Graph Attention Networks},'' in
  \emph{ICLR}, 2018.

\bibitem{xu2019powerful}
K.~Xu \emph{et~al.}, ``How powerful are graph neural networks?'' in
  \emph{International Conference on Learning Representations (ICLR)}, 2019.

\bibitem{topk}
H.~Gao and S.~Ji, ``Graph u-nets,'' in \emph{Proceedings of the 36th
  International Conference on Machine Learning}, 2019.

\bibitem{errica2020fair}
F.~Errica \emph{et~al.}, ``A fair comparison of graph neural networks for graph
  classification,'' in \emph{ICLR}, 2020.

\bibitem{qin2022bench}
Y.~Qin, Z.~Zhang, X.~Wang, Z.~Zhang, and W.~Zhu, ``Nas-bench-graph:
  Benchmarking graph neural architecture search,'' \emph{Advances in Neural
  Information Processing Systems}, vol.~35, pp. 54--69, 2022.

\bibitem{defferrard2016convolutional}
M.~Defferrard, X.~Bresson, and P.~Vandergheynst, ``Convolutional neural
  networks on graphs with fast localized spectral filtering,'' \emph{Advances
  in neural information processing systems}, vol.~29, pp. 3844--3852, 2016.

\bibitem{bianchi2021graph}
F.~M. Bianchi, D.~Grattarola, L.~Livi, and C.~Alippi, ``Graph neural networks
  with convolutional arma filters,'' \emph{IEEE Transactions on Pattern
  Analysis and Machine Intelligence}, 2021.

\bibitem{morris2019weisfeiler}
C.~Morris, M.~Ritzert, M.~Fey, W.~L. Hamilton, J.~E. Lenssen, G.~Rattan, and
  M.~Grohe, ``Weisfeiler and leman go neural: Higher-order graph neural
  networks,'' in \emph{Proceedings of the AAAI Conference on Artificial
  Intelligence}, vol.~33, 2019, pp. 4602--4609.

\bibitem{pitfall}
O.~Shchur, M.~Mumme, A.~Bojchevski, and S.~G{\"u}nnemann, ``Pitfalls of graph
  neural network evaluation,'' \emph{Relational Representation Learning
  Workshop, NeurIPS 2018}, 2018.

\bibitem{ogb}
W.~Hu, M.~Fey, M.~Zitnik, Y.~Dong, H.~Ren, B.~Liu, M.~Catasta, and J.~Leskovec,
  ``Open graph benchmark: Datasets for machine learning on graphs,''
  \emph{Advances in neural information processing systems}, vol.~33, pp.
  22\,118--22\,133, 2020.

\bibitem{yang2016revisiting}
Z.~Yang, W.~Cohen, and R.~Salakhudinov, ``Revisiting semi-supervised learning
  with graph embeddings,'' in \emph{International conference on machine
  learning}.\hskip 1em plus 0.5em minus 0.4em\relax PMLR, 2016, pp. 40--48.

\bibitem{NNIB}
\BIBentryALTinterwordspacing
{Microsoft}, ``{Neural Network Intelligence},'' 1 2021. [Online]. Available:
  \url{https://github.com/microsoft/nni}
\BIBentrySTDinterwordspacing

\bibitem{gao2020graph}
Y.~Gao, H.~Yang, P.~Zhang, C.~Zhou, and Y.~Hu, ``Graph neural architecture
  search,'' in \emph{Proceedings of the Twenty-Ninth International Joint
  Conference on Artificial Intelligence}, vol.~20, 2020, pp. 1403--1409.

\bibitem{li2020random}
L.~Li and A.~Talwalkar, ``Random search and reproducibility for neural
  architecture search,'' in \emph{Uncertainty in artificial
  intelligence}.\hskip 1em plus 0.5em minus 0.4em\relax PMLR, 2020, pp.
  367--377.

\bibitem{yuan2020explainability}
H.~Yuan \emph{et~al.}, ``Explainability in graph neural networks: A taxonomic
  survey,'' \emph{arXiv:2012.15445}, 2020.

\bibitem{li2021oodgnn}
H.~Li, X.~Wang, Z.~Zhang, and W.~Zhu, ``Ood-gnn: Out-of-distribution
  generalized graph neural network,'' \emph{arXiv:2112.03806}, 2021.

\bibitem{li2022out}
------, ``Out-of-distribution generalization on graphs: A survey,'' \emph{arXiv
  preprint arXiv:2202.07987}, 2022.

\bibitem{li2022learning}
H.~Li, Z.~Zhang, X.~Wang, and W.~Zhu, ``Learning invariant graph
  representations for out-of-distribution generalization,'' \emph{Advances in
  Neural Information Processing Systems}, vol.~35, pp. 11\,828--11\,841, 2022.

\bibitem{li2023invariant}
------, ``Invariant node representation learning under distribution shifts with
  multiple latent environments,'' \emph{ACM Transactions on Information
  Systems}, vol.~42, no.~1, pp. 1--30, 2023.

\bibitem{sun2018adversarial}
L.~Sun \emph{et~al.}, ``Adversarial attack and defense on graph data: A
  survey,'' \emph{arXiv:1812.10528}, 2018.

\bibitem{xie2019exploring}
S.~Xie \emph{et~al.}, ``Exploring randomly wired neural networks for image
  recognition,'' in \emph{ICCV}, 2019.

\bibitem{zhang2018graph}
C.~Zhang, M.~Ren, and R.~Urtasun, ``Graph hypernetworks for neural architecture
  search,'' in \emph{ICLR}, 2018.

\bibitem{dudziak2020brp}
L.~Dudziak \emph{et~al.}, ``Brp-nas: Prediction-based nas using gcns,''
  \emph{NeurIPS}, 2020.

\bibitem{qin2021GQNAS}
Y.~Qin, X.~Wang, P.~Cui, and W.~Zhu, ``Gqnas: Graph q network for neural
  architecture search,'' in \emph{ICDM}, 2002.

\bibitem{auten2020hardware}
A.~Auten, M.~Tomei, and R.~Kumar, ``Hardware acceleration of graph neural
  networks,'' in \emph{DAC}, 2020.

\bibitem{cai2018proxylessnas}
H.~Cai, L.~Zhu, and S.~Han, ``Proxylessnas: Direct neural architecture search
  on target task and hardware,'' in \emph{International Conference on Learning
  Representations}, 2018.

\bibitem{tan2019mnasnet}
M.~Tan \emph{et~al.}, ``Mnasnet: Platform-aware neural architecture search for
  mobile,'' in \emph{CVPR}, 2019.

\bibitem{jiang2020hardware}
Y.~Jiang, X.~Wang, and W.~Zhu, ``Hardware-aware transformable architecture
  search with efficient search space,'' in \emph{ICME}, 2020.

\bibitem{dwivedi2020benchmarking}
V.~P. Dwivedi \emph{et~al.}, ``Benchmarking graph neural networks,''
  \emph{arXiv:2003.00982}, 2020.

\bibitem{ying2019bench}
C.~Ying \emph{et~al.}, ``Nas-bench-101: Towards reproducible neural
  architecture search,'' in \emph{ICML}, 2019.

\end{thebibliography}

